Uncovering Sparse Financial Networks with Information Criteria

Empirical measures of financial connectedness based on Forecast Error Variance Decompositions (FEVDs) often yield dense network structures that obscure true transmission channels and complicate the identification of systemic risk. This paper proposes a novel information-criterion-based approach to uncover sparse, economically meaningful financial networks. By reformulating FEVD-based connectedness as a regression problem, we develop a model selection framework that consistently recovers the active set of spillover channels. We extend this method to generalized FEVDs to accommodate correlated shocks and introduce a data-driven procedure for tuning the penalty parameter using pseudo-out-of-sample forecast performance. Monte Carlo simulations demonstrate the approach's effectiveness with finite samples and its robustness to approximately sparse networks and heavy-tailed errors. Applications to global stock markets, S&P 500 sectoral indices, and commodity futures highlight the prevalence of sparse networks in empirical settings.

==> appd_cholesky.tex <==

\newpage
\section{Discussion on Cholesky Decomposition}

\textcolor{purple}{Memo 1: Simulation studies indicate that the sparsity
pattern of the FEVD network is invariant to variable ordering. Specifically,
let $\boldsymbol{\Theta}$ denote the FEVD matrix obtained from block-diagonal
$\boldsymbol{\Sigma}$ and $\boldsymbol{\Phi}_{l}$. If we replace
$\boldsymbol{\Sigma}$ and $\boldsymbol{\Phi}_{l}$ with $\mathbf{Q}\boldsymbol{\Sigma}\mathbf{Q}'$
and $\mathbf{Q}\boldsymbol{\Phi}_{l}\mathbf{Q}'$, respectively, where
$\mathbf{Q}$ is an arbitrary permutation matrix, to calculate the
corresponding FEVD matrix $\tilde{\boldsymbol{\Theta}}$, we observe
that $\mathbf{Q}\mathbf{1}[\boldsymbol{\Theta}=0]\mathbf{Q}'=\mathbf{1}[\tilde{\boldsymbol{\Theta}}=0]$.
This observation, combined with Lemma B.2 and Corollary B.3, implies
that our FEVD network sparsity is invariant to variable ordering.
The implication is that the structural information revealed by the
FEVD network's sparsity is robust to changes in variable ordering,
which is a desirable property. Is it worthwhile to formally prove
this observation? My attempts have suggested that the proof would
be quite tedious and lengthy. Given the simulation evidence and the
support from Lemma B.2 and Corollary B.3, formal proof may offer limited
additional insight. However, we do not have analogous results for
the element values of the FEVD matrix, not surprising.}

\textcolor{purple}{Memo 2: This discussion justifies the use of the
Cholesky decomposition in constructing FEVDs. We show that when the
coefficient and error covariance matrices exhibit a clear clustering
structure, the FEVDs obtained using Cholesky decomposition preserves
their sparsity.}

%\textcolor{purple}{Memo 2: This discussion justifies the use of the Cholesky decomposition in constructing FEVDs. We show that when the coefficient and error covariance matrices exhibit a clear clustering structure, the FEVDs obtained using Cholesky decomposition preserves their sparsity.}

\textcolor{purple}{Memo 3: In this paper, connectedness is defined
in terms of the ``causal'' (Granger?) relationship between $\xi_{t}=P^{-1}\varepsilon_{t}$
and $Y_{t+H}$ from an MA perspective. This differs from the notion
of connectedness in previous literature, which is typically defined
from a VAR perspective as the relationship between $Y_{t,i}$ and
$Y_{t+H,j}$. The discussion here provides sufficient conditions under
which these two perspectives can coincide (in terms of detecting cluster
structure).}

In this section, we assume all matrices are real. The following lemma
establishes the uniqueness of the Cholesky decomposition for positive
definite matrices.

\begin{lemma} \label{lemma:Chol_unique} Let $\boldsymbol{\Sigma}$
be a real $m\times m$ positive definite matrix. Then, 
\begin{enumerate}
\item[(1)] $\boldsymbol{\Sigma}$ admits a unique $\mathbf{U}'\mathbf{D}\mathbf{U}$
decomposition, i.e., $\boldsymbol{\Sigma}=\mathbf{U}'\mathbf{D}\mathbf{U}$,
where $\mathbf{U}$ is a unit upper triangular matrix and $\mathbf{D}$
is a diagonal matrix with positive diagonal elements. 
\item[(2)] $\boldsymbol{\Sigma}$ has a unique Cholesky decomposition, i.e.,
there exists a unique lower triangular matrix $\mathbf{P}$ such that
$\boldsymbol{\Sigma}=\mathbf{P}\mathbf{P}'$. In particular, $\mathbf{P}=\mathbf{D}^{1/2}\mathbf{U}'$
and has positive diagonal elements. 
\end{enumerate}
\end{lemma}

\begin{proof} The results in Lemma \ref{lemma:Chol_unique} are well
established. See, e.g., Corollary 14.5.10 and Theorem 14.5.11 of \citet{harville1997}.
\end{proof}

Consider an $m\times m$ positive definite matrix $\boldsymbol{\Sigma}=[\sigma_{ij}]$.
Its Cholesky decomposition, $\boldsymbol{\Sigma}=\mathbf{P}\mathbf{P}'$,
where $\mathbf{P}=[P_{ij}]$ is a lower triangular matrix, can be
computed using the following recursive formulas (see, e.g., (5.16)--(5.19)
of \citet{harville1997}): 
\begin{align}
P_{11} & =\sqrt{\sigma_{11}},\quad P_{jj}=\sqrt{\sigma_{jj}-\sum_{k=1}^{j-1}P_{jk}^{2}},\quad\text{for }j>1,\nonumber \\
P_{i1} & =\sigma_{i1}/P_{11},\quad P_{ij}=\frac{1}{P_{jj}}\left(\sigma_{ij}-\sum_{k=1}^{j-1}P_{ik}P_{jk}\right),\quad\text{for }i>j>1.\label{eq:Chol_formula}
\end{align}

Using these formulas, we can show the following property of Cholesky
decomposition. \begin{lemma} \label{lemma:Chol_0} Let $\boldsymbol{\Sigma}=[\sigma_{ij}]=\textrm{diag}[\boldsymbol{\Sigma}_{1},...,\boldsymbol{\Sigma}_{G}]$
be a block-diagonal, positive definite matrix. Assume that each block
$\boldsymbol{\Sigma}_{g}$, for $g=1,\dots,G$, is fully dense (i.e.,
contains no zero elements). Let $\boldsymbol{\Sigma}$ admit the Cholesky
decomposition $\boldsymbol{\Sigma}=\mathbf{P}\mathbf{P}'$, where
$\mathbf{P}=[P_{ij}]$ is a lower triangular matrix. Then, for all
$i>j$, we have $P_{ij}=0$ whenever $\sigma_{ij}=0$. \end{lemma}

\begin{proof} Let $i>1$. For $j=1$, it follows from (\ref{eq:Chol_formula})
that $\sigma_{i1}=0$ implies $P_{i1}=0$, given that $P_{11}>0$.
We proceed by induction to show that $\sigma_{ij}=0$ implies $P_{ij}=0$
for all $1<j<i$. Assume the statement holds for $j=1,...,l$, where
$l<i-1$. Then, the statement must also hold for column $l+1$. To
see this, applying (\ref{eq:Chol_formula}) yields 
\[
P_{i(l+1)}=\frac{1}{P_{(l+1)(l+1)}}\left[\sigma_{i(l+1)}-\left(P_{i1}P_{(l+1)1}+\cdots+P_{i(l-1)}P_{(l+1)(l-1)}+P_{il}P_{(l+1)l}\right)\right].
\]
If $\sigma_{i(l+1)}=0$, then $\sigma_{i1},...,\sigma_{il}$ must
all be zero because $\boldsymbol{\Sigma}$ is block-diagonal, implying
$P_{i1}=\cdots=P_{il}=0$. Therefore, $P_{i(l+1)}=\sigma_{i(l+1)}/P_{(l+1)(l+1)}=0$.
Thus, the proof is completed, noting that row $i$ was chosen arbitrarily.
\end{proof}

\begin{remark} \label{remark:Chol_counterexample} The converse of
Lemma \ref{lemma:Chol_0} is not generally true. To see this, consider
\[
\boldsymbol{\Sigma}=\begin{bmatrix}\boldsymbol{\Sigma}_{1} & \mathbf{0}\\
\mathbf{0} & \boldsymbol{\Sigma}_{2}
\end{bmatrix}\textrm{ with }\boldsymbol{\Sigma}_{1}=\begin{bmatrix}1 & \frac{1}{2} & \frac{1}{3}\\
\frac{1}{2} & 1 & \frac{1}{6}\\
\frac{1}{3} & \frac{1}{6} & 1
\end{bmatrix}.
\]
By Lemma \ref{lemma:Chol_unique}, there exist unique lower triangular
matrices $\mathbf{P}_{1}$ and $\mathbf{P}_{2}$ such that $\boldsymbol{\Sigma}_{1}=\mathbf{P_{1}}\mathbf{P_{1}}'$
and $\boldsymbol{\Sigma}_{2}=\mathbf{P_{2}}\mathbf{P_{2}}'$. Define
the lower triangular matrix $\mathbf{P}=\textrm{diag}[\mathbf{P}_{1},\mathbf{P}_{2}]$.
Then, by uniqueness, 
\[
\boldsymbol{\Sigma}=\begin{bmatrix}\boldsymbol{\Sigma}_{1} & \mathbf{0}\\
\mathbf{0} & \boldsymbol{\Sigma}_{2}
\end{bmatrix}=\begin{bmatrix}\mathbf{P}_{1} & \mathbf{0}\\
\mathbf{0} & \mathbf{P}_{2}
\end{bmatrix}\begin{bmatrix}\mathbf{P}_{1}' & \mathbf{0}\\
\mathbf{0} & \mathbf{P}_{2}'
\end{bmatrix}=\mathbf{P}\mathbf{P}'
\]
is the Cholesky decomposition of $\boldsymbol{\Sigma}$.\footnote{This also provides an alternative proof of Lemma \ref{lemma:Chol_0}.}
However, direct calculation yields 
\[
\mathbf{P}_{1}=\begin{bmatrix}1 & 0 & 0\\
\frac{1}{2} & \frac{\sqrt{3}}{2} & 0\\
\frac{1}{3} & 0 & \frac{2\sqrt{2}}{3}
\end{bmatrix}.
\]
Notice that $P_{32}=0$, but $\sigma_{32}=1/6\neq0$. This provides
a counterexample, demonstrating that for $i>j$, $P_{ij}=0$ does
not necessarily imply $\sigma_{ij}=0$. \end{remark}

\begin{remark} Despite the counterexample in Remark \ref{remark:Chol_counterexample},
a careful examination of (\ref{eq:Chol_formula})---by expressing
each $P_{ij}$ as a function of $\sigma_{ij}$’s---suggests that
the event $\{P_{ij}=0,\sigma_{ij}\neq0,i>j\}$ occurs only when $\sigma_{ij}$’s
satisfy a complex system of recursive nonlinear equations, which lacks
a meaningful interpretation. Thus, the counterexample is of purely
mathematical interest, and such events are unlikely to occur in practice.

To verify this intuition, we conduct a small-scale Monte Carlo simulation.
We randomly generate $\boldsymbol{\Sigma}_{1}$ and $\boldsymbol{\Sigma}_{2}$,
with their dimensions drawn from a discrete uniform distribution over
$\{2,\dots,9\}$. Using the same method as in \textcolor{purple}{Section
X} to construct error covariance matrices, we ensure they satisfy
all conditions in Lemma 2, then assemble the block-diagonal positive
definite matrix $\boldsymbol{\Sigma}=\textrm{diag}[\boldsymbol{\Sigma}_{1},\boldsymbol{\Sigma}_{2}]$.
We then compute its Cholesky decomposition, $\boldsymbol{\Sigma}=\mathbf{P}\mathbf{P}'$,
and count the occurrences of the event $\{P_{ij}=0,\sigma_{ij}\neq0,i>j\}$.
Across one million independent replications, this event never occurs.
Thus, although Lemma \ref{lemma:Chol_0} does not establish a strict
``if and only if'' result, our findings suggest that, in practice,
the Cholesky decomposition preserves the sparsity of $\boldsymbol{\Sigma}$
satisfying the conditions of Lemma \ref{lemma:Chol_0}---that is,
for all $i>j$, $\sigma_{ij}=0$ if and only if $P_{ij}=0$. \end{remark}

\begin{corollary} If $\boldsymbol{\Phi}_{l}=[\phi_{l,ij}]$ for $l=1,\dots,p$
have the same block-diagonal structure as $\boldsymbol{\Sigma}$ and
satisfy all conditions for $\boldsymbol{\Sigma}$ in Lemma \ref{lemma:Chol_0},
except for positive definiteness, then $\varphi_{ij}=0$ for all $(i,j)$
that do not belong to any block. \end{corollary}

\begin{proof} It suffices to consider the case with two blocks, i.e.,
\[
\boldsymbol{\Phi}_{l}=\begin{bmatrix}\boldsymbol{\Phi}_{l1} & \mathbf{0}\\
\mathbf{0} & \boldsymbol{\Phi}_{l2}
\end{bmatrix},\quad\boldsymbol{\Sigma}=\begin{bmatrix}\boldsymbol{\Sigma}_{1} & \mathbf{0}\\
\mathbf{0} & \boldsymbol{\Sigma}_{2}
\end{bmatrix}=\mathbf{P}\mathbf{P}',
\]
where $\mathbf{P}$ is lower triangular. By construction and the derivation
in Remark \ref{remark:Chol_counterexample}, $\boldsymbol{\Psi}_{h}$
and $\mathbf{P}$ also have a block-diagonal structure: 
\[
\boldsymbol{\Psi}_{h}=\begin{bmatrix}\boldsymbol{\Psi}_{h1} & \mathbf{0}\\
\mathbf{0} & \boldsymbol{\Psi}_{h2}
\end{bmatrix},\quad\mathbf{P}=\begin{bmatrix}\mathbf{P}_{1} & \mathbf{0}\\
\mathbf{0} & \mathbf{P}_{2}
\end{bmatrix}.
\]
Since all relevant matrices preserve the block-diagonal structure,
the result follows. \end{proof}
